Exploring Privacy Preservation in Outsourced K-Nearest Neighbors with Multiple Data Owners

The k-nearest neighbors (k-NN) algorithm is a popular and effective classification algorithm. Due to its large storage and computational requirements, it is suitable for cloud outsourcing. However, k-NN is often run on sensitive data such as medical records, user images, or personal information. It is important to protect the privacy of data in an outsourced k-NN system. Prior works have all assumed the data owners (who submit data to the outsourced k-NN system) are a single trusted party. However, we observe that in many practical scenarios, there may be multiple mutually distrusting data owners. In this work, we present the first framing and exploration of privacy preservation in an outsourced k-NN system with multiple data owners. We consider the various threat models introduced by this modification. We discover that under a particularly practical threat model that covers numerous scenarios, there exists a set of adaptive attacks that breach the data privacy of any exact k-NN system. The vulnerability is a result of the mathematical properties of k-NN and its output. Thus, we propose a privacy-preserving alternative system supporting kernel density estimation using a Gaussian kernel, a classification algorithm from the same family as k-NN. In many applications, this similar algorithm serves as a good substitute for k-NN. We additionally investigate solutions for other threat models, often through extensions on prior single data owner systems.

==> discussion.tex <==
\section{Discussion}

\subsection{Performance Overhead}

In this paper, we have provided an initial exploration of privacy preservation in a multi-data owner k-NN system. In particular, we have provided a kernel density solution for the DO-Q threat model, and extensions on existing schemes for other threat models. However, both our kernel density solution as well as the cited existing schemes require $O(N)$ computation and communication overhead, where $N$ is the number of data tuples in the data set. 

One solution for increasing performance is parallelism, since our scheme operates on each data tuple independent of other tuples. Ideally, multiple machines would run in parallel at both cloud parties, providing parallelism not only in computation but also network communication. Each machine at the data host would compute a subcomponent of the classification influence vector, and one master node can aggregate these into the final classification answer vector returned to queriers.

K-NN suffers this linear-growth complexity as well, however approximation algorithms significantly improve performance by reducing the number of points considered during neighbor search. For example, k-d trees divide the search space into smaller regions, while locality hashing hashes nearby points to the same bin. Hence, search for a query's neighbor involves computation over the data points in the same region or bin, rather than the entire data set.
Unfortunately, it is not obvious how to execute approximate k-NN in a privacy preserving fashion. Some party in the k-NN system must determine the mapping of tuples to bins/regions, and thus recovers some bits of an encrypted tuple based on observed mappings. In certain applications, the privacy tradeoff for performance increase may be acceptable. An investigation into privacy preserving systems for such applications remains for future work.



\subsection{Alternative Defenses}

This paper introduce a novel and privacy preserving kernel density estimation outsourced system as an alternative to the insecure outsourced k-NN system under the DO-Q threat model. However, there are alternative defense approaches. One is noise, where data tuples and queries can be perturbed such that the original values are protected. This approach may impact the accuracy of kNN since data points are now incorrect (however slight), and only protects values up to a probability distribution (e.g. knowing the noise formulation can reveal the probability distribution of the true value). Hence we did not focus on noise defenses in this work. However, an analysis of its accuracy versus privacy guarantees compared with those of the kernel density system is worthwhile, and we leave that for future work.

Another defense approach is in the field of detection and mitigation. The distance-learning attacks may follow a particular pattern that can be detected by cloud providers. Granted, this approach will not work given a misbehaving cloud provider, but is certainly worth exploration. We have not been able to design an adequate solution in this regard.

One method we attempted involved tracking potential attacks on data tuples, and flagging those  that may have been compromised. We observed that if an attack uses a query $q$ at distance $d$ from a target tuple $t$,  the attacker must insert at least one guess tuple within distance $d$ of $q$. The method aimed to detect such behavior. We believe tracking all queries over time is prohibitively expensive, so instead we monitor the behavior with relations to the data tuples. The guess tuple is at most distance $2d$ from $t$. Hence, a conservative hypersphere of radius $2d$ can surround $t$ and be designated as a potential attack space. Any insertions within this radius is flagged, and in a $k$-dimensional space, $k$ flagged attacks mean $t$ may be compromised. To prevent data privacy breach, we simply removed the potentially compromised points. Unfortunately, this defense does not perform well because benign insertions can easily result in many removals of data tuples, because each insertion may be in multiple data tuples' attack space. We are investigating other techniques for future work.

